A Spline-Based Collocation Method for Stokes and Navier-Stokes equations

In the paper, we propose a collocation method based on multivariate polynomial splines over triangulation or tetrahedralization for solving Stokes and Navier-Stokes equations. We start with a detailed explanation of the method for the Stokes equation and then extend the study to the Navier-Stokes equations. We shall show that the numerical solution can approximate the exact PDE solution very well over several domains. Then we present several numerical experimental results to demonstrate the performance of the method over the 2D and 3D settings. Also, we apply the IPBM method to our method to find the solution over several curved domains effectively. In addition, we present a comparison with the existing multivariate spline methods in \cite{AL02} and several existing methods to show that the new method produces a similar and sometimes more accurate approximation in a more efficient fashion.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{  A Spline-Based Collocation Method for Stokes and Navier-Stokes equations}{Jinsil Lee}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{  A Spline-Based Collocation Method for Stokes and Navier-Stokes equations\thanks{Submitted to the editors DATE.
\funding{This work was funded by NRF-2019R1A6A1A11051177.}}}

% Authors: full names plus addresses.
\author{Jinsil Lee\thanks{ Department of Mathematics, Ewha W. University, Seoul 120-750, South Korea
		(\email{jl74942@ewha.ac.kr})}
}
	
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

